Least angle and $\ell_1$ penalized regression: A review

Least Angle Regression is a promising technique for variable selection applications, offering a nice alternative to stepwise regression. It provides an explanation for the similar behavior of LASSO ($\ell_1$-penalized regression) and forward stagewise regression, and provides a fast implementation of both. The idea has caught on rapidly, and sparked a great deal of research interest. In this paper, we give an overview of Least Angle Regression and the current state of related research.

==> computation.tex <==
\subsection{Computational Issues}
\label{section.computation}

There are three primary computation issues:  speed, memory usage,
and numerical accuracy.

% numerical accuracy
% 
% dependent variables
% 
% memory usage
% 
% speed


The original LAR algorithm for linear regression
as described in \cite{efro04} and implemented in 
\cite{efro03}\footnote{S-PLUS and R package \texttt{lars} is available.} is remarkably fast 
and memory efficient in the $p < n$ case,
as noted in Section~\ref{section.significance}.
Minor modifications allow computing the LASSO and forward stagewise cases.
However, the implementations use cross-product matrices, 
which are notorious for numerical
inaccuracy with highly correlated predictors.

\nocite{hest06d,hest06c}
\cite{fral07} (see also Hesterberg and Fraley 2006a,b)
develop LARS
implementations based on $QR$ decompositions
\footnote{S-PLUS and R package \texttt{sclars} is available.}.
This reduces the roundoff error by a factor
equal to the condition number of $X$ relative to the original
algorithm.
% \fbox{same order of operation count?}
One variation uses only a single pass through the data for an initial 
factorization, after which it requires storage $O(p^2)$, independent of $n$;
in contrast the original LARS implementation 
is intended for in-memory datasets, and makes multiple passes through the data.
% four for centering and scaling x,
% two for centering y, 
% one for Cvec
% one for ssy
% two for computing residuals

\citet{fu98} proposes a shooting algorithm to solve LASSO
for a specified value of the penalty parameter $\theta$. The algorithm
is a special case of a coordinate descent method that cycles through
the coordinates, optimizing the current one and keeping the
remaining coordinates fixed. Using a (predefined) grid of penalty
parameters, the coefficient paths can be computed efficiently,
especially in very high-dimensional settings, by making use of the
preceding solution as starting values. 

Other coordinate-wise optimization
techniques have shown their success with other penalty types and also
for nonlinear models
(\citealt{genkin07}; \break\citealt{yuan06,meie08,frie07c,frie07d}).

\citet{osbo00} propose a descent algorithm for a LASSO problem with a
specified value of the penalty parameter $\theta$, as well as a homotopy
method for the piecewise linear solution path in the linear regression
case that is related to the LAR implementation of \cite{efro04}.
In \cite{osbo00b}, an algorithm based on LASSO and its
dual is proposed that yields new insights and an improved method for
estimating standard errors of regression parameters.

\paragraph{Nonlinear regression}

In the linear
regression case the solution path is piecewise linear, and each
step direction and jump size can be computed in closed-form solution.
In the nonlinear case paths are curved, so that iterative methods
are needed for computing and updating directions and determining
the ends of each curve, requiring
multiple passes through the data.  Hence the algorithms are much
slower than in the linear case.


% \fbox{Write more?}
% Can we say anything about particularly effective strategies
% in the literature?


% --------------------------------------------------

% From Phase II proposal:
%
% We developed a more accurate algorithm for the linear case,
% using the $QR$ decomposition of $X$ rather than the Cholesky
% decomposition of cross-product matrices $X'X$.  For example,
% with $n=100$, $p=50$, and correlation 0.999999 between each pair
% of predictors, the new algorithm has mean absolute roundoff error
% of $7.5\times10^{-13}$, compared to $1.8\times10^{-8}$ for the
% original algorithm.  The ratio between these numbers is 24346,
% approximately equal to the condition number of $X$, 21760, as
% expected.  Note that in practice it is easy to get even higher
% condition numbers even with lower pairwise correlations, due
% to higher-dimensional collinearity.
% 
% The more accurate algorithm is slower than the original
% ($\sim$4.8 times slower),
% in the current S implementation.  Converting this to
% FORTRAN or some other compiled language 
% should result in a substantial speedup, even more than
% the factor of 16 observed for the other algorithm, 
% because we could use $QR$ updating techniques when adding or dropping
% variables, whereas the prototype
% S implementation recomputes the decomposition from scratch in each step.
% We expect the ultimate speed to nearly equal the original algorithm.
% 
% We also made advances in an area related
% to accuracy, but not anticipated in the Phase~I proposal ---
% linear dependence.  When predictors are linearly dependent
% then an ordinary linear least squares fit is ill-defined, unless
% predictors are dropped from the model.  Similar, in LARS, the set
% of active variables should not be linearly dependent.  
% Our software checks for linear dependence, and excludes dependent
% inactive variables from consideration for activation, permanently
% in the LAR case, and temporarily in the LASSO case
% (when a variable leaves a model, the set of variables that should
% be prohibited may change).




% LocalWords:  efro fu genkin meie friedman pathwise osbo


==> future_work.tex <==
\section{Conclusions and Future Work}

%\paragraph{Turning promise into practice}

LARS has considerable promise, offering speed, interpretability,
relatively stable predictions, nearly unbiased inferences,
and a nice graphical presentation of coefficient paths.
%of the whole sequence of coefficients.
But considerable work is required in order to realize
this promise in practice.
%\begin{squeezeitemize}
%\item
A number of different approaches have been suggested, both for 
linear and nonlinear models; 
further study is needed to determine their advantages and drawbacks.
Also various implementations of some of the approaches have
been proposed that differ in speed, numerical stability, and
accuracy; these also need further assessment.
% These differ in speed, numerical stability, 
% accuracy (in the nonlinear case, how
% well do algorithms track the exact curved coefficient paths), 
% collinearity, and handling
% of details such as variables that are nearly tied in importance.
%Additional algorithms are undoubtedly being developed.  
%Work is needed to compare the algorithms, with artificial and real data,
%with a variety of sizes --- large and small $n$ and $p$.

%\item
Alternate penalties such as the elastic net 
and fused LASSO have  advantages for certain kinds of data 
(e.g.\ microarrays and proteomics).
The original LARS methodology is limited to continuous or binary covariates;
grouped LASSO and LAR offer an extension to factor variables
or other variables with multiple degrees of freedom such as polynomial
and spline fits.  
Work is needed to further investigate the properties of these methods,
%to provide guidance in choosing tuning parameters,
and to extend them to nonlinear models.

%\item
Further work is also needed to address some practical considerations,
including order restrictions
(e.g.~main effects should be included in a model before interactions,
or linear terms before quadratic),
forcing certain terms into the model,
allowing unpenalized terms,
or applying different levels of penalties to different predictors
based on an analyst's knowledge.
For example, when estimating a treatment effect, the treatment term
should be forced into the model and estimated without penalty, while
covariates should be optional and penalized.

Additional work is needed on choosing tuning parameters such as
the magnitude of the $\Lone$ penalty parameter in LASSO and other methods,
the number of steps for LAR, and the multiple tuning parameters for elastic
net and fused LASSO.
Closely related is the question of
statistical inference: is a larger model significantly better than
a simpler model?
Work is needed to investigate and compare model-selection methods including
$C_p$, AIC, BIC, cross-validation, and empirical Bayes.


%\item
Work is also needed to develop estimates of bias, standard error, and
confidence intervals, for predictions, coefficients, and
linear combinations of coefficients.
Are predictions sufficiently close to normally-distributed to
allow for the use of $t$ confidence intervals?  
Does it even make sense to compute standard errors?
Coefficients are
definitely not normally distributed, due to a point mass at zero;
but when coefficients are sufficiently large, might $t$ intervals
still be useful, and how would one compute the standard errors?

%\item
The signal-to-noise ratio needs to be examined for the proposed methods, 
and alternatives compared.  
Evidence for a good signal-to-noise ratio would provide a strong impetus 
for their adoption by the statistical community.

Speed is also an issue, particularly for nonlinear models, 
and especially when
cross validation is used for model selection or bootstrapping is used
for inferences.
In the linear regression case the cross-product matrices or $QR$
decomposition required for computations
can be calculated in a single pass through the data.
%and all computations performed from either summary of the data.
In contrast, for nonlinear models, fitting each
subset of predictors requires multiple passes.
Development of fast methods for nonlinear models is highly desirable.

%\item
Finally, to truly realize the promise of these methods
beyond the domain of academic research,
work is needed on usability issues.
Implementations must be robust, 
numerical and graphical diagnostics
to interpret regression model output must be developed,
and interfaces must be targeted to a broad base of users.
%\end{squeezeitemize}

%--------------------------------------------------

We close on a positive note, with
comments in the literature about LARS:
\cite{knig04}
is impressed by the robustness of LASSO to small changes in its
tuning parameter, relative to more classical stepwise subset selection
methods, and notes
``What seems to make the LASSO special
is (i) its ability to produce exact 0 estimates and (ii) the `fact' that its
bias seems to be more controllable than it is for other methods (e.g., ridge
regression, which naturally overshrinks large effects) \ldots''
\cite{loub04} indicate
``It seems to us that it solves practical questions of crucial interest
and raises very interesting theoretical questions \ldots''.
\cite{sega03} write
``The development of least angle regression (LARS) \citeP{efro04}
which can readily be specialized to provide all LASSO solutions in a
highly efficient fashion, represents a major breakthrough. LARS is a
less greedy version of standard forward selection schemes. The simple
yet elegant manner in which LARS can be adapted to yield LASSO
estimates as well as detailed description of properties of procedures,
degrees of freedom, and attendant algorithms are provided by
\cite{efro04}.''

The procedure has enormous potential, which is evident in the amount
of effort devoted to the area by such a large number of authors in the short
time since publication of the seminal paper.  We hope that
this article provides a sense of that value.

Additional information, including software, may be found at\break
\url{www.insightful.com/lars} 
% {\tt www.insightful.com/Hesterberg/glars}.
% Unfortunately, \usepackage{hyperref} does not appear to be compatible
% with the bibtex routines we're using. (no longer true)



% LocalWords:  rrrrrrrrrrrr BMI BP efro Z'Z X'X X'Y Y'X Y'Y kenn lang mona drap
% LocalWords:  tibs ABD osbo gui madi ross EHJT lokh brdgrun wu glmpath glasso
% LocalWords:  kim GLARS Rosset Ji Saharon Mee Suhrid Balakrishnan Ridgeway Zou
% LocalWords:  Weisberg Leming Qu Peng Zhao Guilherme Yu Jiang Efroymson's cov
% LocalWords:  zhu IRLS sega zou interpretability overshrinks fu Massart GPL
% LocalWords:  Efron's elasticnet Amgen AIC BIC overfits reweighted biotech
% LocalWords:  microrarrays Zamar Aelst ishw loub stin vana


==> general_problem.tex <==
\section{LARS Extensions}
\label{section.related}

In this section we review extensions to LARS and other contributions
described in the literature.  
We introduce LARS extensions that account for specific structures in
variables
in Section~\ref{section.structure}, 
extensions to nonlinear models in
Section~\ref{section.nonlinear},
extensions in other settings
in Section~\ref{section.otherapp},
and computational issues in
Section~\ref{section.computation}.

% create a section for Future work??

% \subsection{Alternate Regularization Approaches}
Ridge regression and LASSO optimize a criterion that includes
a penalty term.  A number of authors develop other penalty approaches,
including SCAD \citeP{fan01}, adaptive LASSO \citeP{zou06},
relaxed LASSO \citeP{mein07a}, and 
the Dantzig selector \citeP{cand07}.
Some of these may be considered as alternatives rather than extensions
to LARS, so we defer this discussion until
Section~\ref{section.alternateRegularization}.


% LocalWords:  zou mein cand


==> other_applications.tex <==
\subsection{Other Applications}
\label{section.otherapp}

\paragraph{Robust Regression}

\cite{ross04b} and \cite{owen06} extend LASSO by replacing the squared error loss
by Huber's loss.  In the linear regression case this also yields
piecewise-linear solution paths, allowing for fast solutions.
\cite{vana05u} extend LAR by replacing correlations with robust
correlation estimates.

\paragraph{Subset of Observations}
%% applications
LARS can be used for choosing an important subset of observations as
well as for selecting a subset of variables.  \cite{silv05} apply LARS
for selecting a representative subset of the data for use as
landmarks to reduce computational
expense in nonlinear manifold models.


\paragraph{Principal Component and Discriminant Analysis}
%The idea of using $\Lone$ penalty is borrowed by Principal Component
%Analysis (PCA) and other settings.  Derived variables (principal
%components) in PCA are linear combinations of all variables.  People
%usually ignore small coefficients in the principal components, and
%interpret them based on larger coefficients.  But if substantial
%proportion of variables in a principal component have nontrivial
%coefficients, it is hard to make a useful interpretation about the
%component.  
\cite{joll03} and \cite{zou06b} apply $\Lone$ penalties to get
sparse loadings in principal components.  \cite{tren07} discuss
$\Lone$ penalties in linear discriminant analysis.

\paragraph{Gaussian Graphical Models}
A number of authors discuss using $\Lone$ penalties to estimate a
sparse inverse covariance matrix (or a sparse graphical model).
\cite{mein06lasso} fit a LASSO model to each variable, using
the others as predictors, then set the $ij$ term of the inverse
covariance matrix to zero if the coefficient of $X_j$ for predicting
$X_i$ is zero, or the converse.
Many authors
\citep{yuan07a,bane07,dahl07,yuan07b,frie07d}
discuss efficient methods for optimizing the $\Lone$-penalized
likelihood, using interior-point or blockwise coordinate-descent
approaches. This work has yet to be extended to handle nonlinear
relationships between variables, such as (\ref{eqn.basis}).


==> software.tex <==
\section{Software}
\label{section.software}

There are a number of {\tt S-PLUS} and {\tt R} packages related to LARS, 
including:
\texttt{brdgrun} \citeP{fu00},
\texttt{elasticnet} \citeP{zou05c},
\texttt{glars}\break \citeP{hest06b},
\texttt{glasso} \citeP{kim05b},
\texttt{glmpath}\break \citeP{park06b},
\texttt{grplasso} \citeP{meie08},
\texttt{lars} \citeP{efro03},
\texttt{lasso2} \citeP{lokh99},
\texttt{relaxo} \citeP{mein07a}.
%\texttt{mboost} \citeP{buhl07b}.
%\fbox{Nam Hee, add to this list.}

